KappaFace: Adaptive Additive Angular Margin Loss for Deep Face Recognition

Feature learning is a widely used method employed for large-scale face recognition. Recently, large-margin softmax loss methods have demonstrated significant enhancements on deep face recognition. These methods propose fixed positive margins in order to enforce intra-class compactness and inter-class diversity. However, the majority of the proposed methods do not consider the class imbalance issue, which is a major challenge in practice for developing deep face recognition models. We hypothesize that it significantly affects the generalization ability of the deep face models. Inspired by this observation, we introduce a novel adaptive strategy, called KappaFace, to modulate the relative importance based on class difficultness and imbalance. With the support of the von Mises-Fisher distribution, our proposed KappaFace loss can intensify the margin's magnitude for hard learning or low concentration classes while relaxing it for counter classes. Experiments conducted on popular facial benchmarks demonstrate that our proposed method achieves superior performance to the state-of-the-art.

==> Sections/4_experimental_resutls.tex <==
\section{Experimental results}
\subsection{Implementation Details}

\textbf{Datasets.} We utilize the MS1MV2   \cite{deng2019arcface} as our training set to ensure a fair comparison with other prior state-of-the-art methods. MS1MV2 contains approximately 5.8M images of 85,742 identities. We perform computationally extensive experiments on several popular benchmarks, namely LFW \cite{huang2008labeled}, CFP-FP   \cite{sengupta2016frontal}, CPLFW   \cite{zheng2018cross}, AgeDB   \cite{moschoglou2017agedb}, CALFW   \cite{zheng2017cross}, YTF \cite{whitelam2017iarpa}, IJB-B   \cite{whitelam2017iarpa}, IJB-C   \cite{maze2018iarpa}, and MegaFace Challenge 1 \cite{kemelmacher2016megaface}.


\textbf{Training Setting.} For data pre-processing, we follow  ArcFace \cite{deng2019arcface} and obtain the normalized face crops (112 × 112) by utilizing five landmarks \cite{zhang2016joint, tai2019towards}. For the embedding network, we adopt ResNet100 as reported in   \cite{deng2019arcface}. We train models on NVIDIA GeForce RTX 3090 Ti with a batch size of 512. The models are trained using Stochastic Gradient Descent (SGD) algorithm, with the momentum parameter of 0.9 and the weight decay of $5e - 4$. We divide the learning rate at 10, 18, and 22 epochs, and finish at 24 epochs. Regarding the memory buffer, we set the momentum parameters $\alpha = 0.3$ and $m=0.999$, whereas $\gamma$ is set to 0.7. Also, we fix the initial margin value for~\SystemName~(\textbf{\texttt{Momentum encoder}}) for a couple of epochs to avoid {convergence failure}. All experiments are implemented using PyTorch \cite{paszke2019pytorch, insightface}. Additionally, we utilize Partial FC \cite{an2020partical_fc}, which is a sparse variant of the model parallel architecture for large scale face recognition.

\subsection{Evaluation Results}

\begin{table*}[t!]
\begin{center}
\caption{Verification performance, in terms of accuracy, results (\%) on LFW, YTF, two pose benchmarks (CFP-FP and CPLFW), and two age benchmarks (AgeDB and CALFW). }
\label{tb:main_exp}
\resizebox{.780\textwidth}{!}{%
    \begin{tabular}{ l|c|c|c|c|c|c} 
    \Xhline{3\arrayrulewidth}
    Method & LFW & CFP-FP & CPLFW & AgeDB & CALFW & YTF\\
    \hline \hline
    Center Loss  \cite{wen2016discriminative} & 99.27 & - & 81.40 & - & 90.30 & 94.9\\
    SphereFace \cite{liu2017sphereface} & 99.27 & - & 81.40 & - & 90.30 &95.0\\
    VGGFace2  \cite{VGGFace2} & 99.43 & - & 84.00 & - & 90.57 &-\\ 
    UV-GAN  \cite{deng2018uv} & 99.60 & 94.05 & - & - & - & -\\
    ArcFace  \cite{deng2019arcface} & \underline{99.82} & 98.27 & 92.08 & 98.15 & 95.45 & 98.0\\
    
    % BroadFace \cite{kim2020broadface}& \textbf{99.85} & 98.63 & 93.17 &98.38 &96.20 &98.0 \\
    ArcFace-SCF   \cite{li2021spherical} & \underline{99.82} & 98.40 & 93.16 & 98.30 & 96.12 & -\\
    CurricularFace  \cite{huang2020curricularface}  & 99.80 & 98.37 & 93.13 & 98.32 & \underline{96.20} & -\\
    % AdaFace $^\diamondsuit$ \cite{kim2022adaface} & \underline{99.82} & 98.53 & \textbf{93.47} & 98.17 & 96.02 & -\\
    MagFace \cite{meng2021magface} & \textbf{99.83} & 98.46 & 92.87 & 98.17 & 96.15 & -\\
    % AdaFace \cite{kim2022adaface} & \underline{99.82} & 98.49 & \textbf{93.53} & 98.05 & 96.08 & -\\
    
    \hline
    KappaFace (\textbf{\texttt{Memory buffer}}) & \textbf{99.83} & \textbf{98.69} & \underline{93.22} & \textbf{98.47} & \textbf{96.23}  & \textbf{98.0}\\
        KappaFace (\textbf{\texttt{Momentum encoder}}) & \textbf{99.83} & \underline{98.60} & \textbf{93.40} & \underline{98.35} & {96.15}  & \textbf{98.0}\\
    \Xhline{3\arrayrulewidth}
    \end{tabular}
    }
\end{center}
\end{table*}

\textbf{Results on LFW, CFP-FP, CPLFW, AgeDB,
CALFW, and YTF.} We train our KappaFace on MS1MV2 using ResNet100 as a backbone and provide a comparison with other SOTA methods. In this paper, we follow the unrestricted with labeled outside data protocol, as in \cite{deng2019arcface, huang2020curricularface}, to report the results. Additionally, we used 7,000 pair testing images for CFP-FP and 6,000 pairs for the rest of the datasets to report our results similar to ArcFace\cite{deng2019arcface}. As shown in Table \ref{tb:main_exp}, our method achieves slightly better results on LFW, YTF and CALFW, where the performance is almost saturated. However, our KappaFace demonstrates a superiority by outperforming counterparts by a significant margin on most of the other datasets, such as CFP-FP, CPLFW and AgeDB, which can be clearly observed from the result table. {The performance on LFW is saturated; however, we still include this benchmark for consistency with previously related works. For the current SOTA methods, the LFW dataset is fairly easy since there is not much variation in terms of identity's facial angles and ages.} 
%Meanwhile, for CPLFW, only AdaFace outperforms KappaFace; however, our method consistently outperforms AdaFace on all other facial benchmarks, which shows the better generalization capability and robustness of KappaFace.} 
Similarly, our proposed method achieves higher accuracy than the ArcFace-SCF \cite{li2021spherical}, which is the SOTA method that also inherits the spherical distribution properties; however, it is applied on individual samples instead. 
% Compared to another memory-based method, namely BroadFace, our ~\SystemName~ mostly dominates the performance across the datasets. 
Additionally, we provide an insight on the concentration values we observed throughout the training process in the ablation studies \textcolor{red}{3}.    
\begin{figure}[t!]
    \centering
    \subfloat[ROC for IJB-B ]{{\includegraphics[width=8.cm]{Figures/ijbb.jpg} }}
    \qquad
    \subfloat[ROC for IJB-C]{{\includegraphics[width=8.cm]{Figures/ijbc.jpg} }}%
    \caption{\textbf{ROC of 1:1 verification protocol on IJB-B and IJB-C}. A comparison of KappaFace
(Memory buffer) and ArcFace on IJB-B and IJB-C, where
our KappaFace demonstrates a superiority over ArcFace even at FAR=$1e^{-6}$.}%
    \label{fig:roc-ijb}%
\end{figure}

\textbf{Results on IJB-B and IJB-C.} The IJB-B dataset consists of 1,845 identities having 21.8K still images and 55K frames collected from 7,011 videos. There are 10,270 positive pairs and 8M negative pairs used for the 1:1 verification. IJB-C is an extension of IJB-B that includes 3,500 subjects with 31K images and 117K frames. There are 19,557 positive pairs and 15,638,932 negative pairs used for the 1:1 verification. Finally, we use our pre-trained KappaFace-MS1MV2-R100 and validate the model on the IJB-B and IJB-C datasets. In Table \ref{tb:ijb_exp}, we provide a comparison in terms of True Acceptance Rate (TAR) (@FAR=$1e^{-4}$) with other state-of-the-art methods. Table~\ref{tb:ijb_exp} demonstrates that KappaFace with the momentum encoder clearly boosts the performance on both datasets by achieving the accuracy of $95.3\%$ and $96.6\%$ on IJB-B and IJB-C, respectively. In Fig. \ref{fig:roc-ijb}, we present the full ROC curves comparing our KappaFace (\textbf{\texttt{Memory buffer}}) and ArcFace on IJB-B and IJB-C, where our KappaFace demonstrates a staggering improvement in performance over ArcFace even at FAR=$1e^{-6}$ establishing a new baseline performance.


\begin{table*}[t!]
\caption{{1:1 verification TAR, measured in \%, (@FAR= $1e^{-4}$) on the IJB-B and IJB-C datasets, where the best performances are shown in bold, and the second best are underlined.}}
\label{tb:ijb_exp}
\begin{center}
\resizebox{.63\textwidth}{!}{%
    \begin{tabular}{ l|c|c} 
    \Xhline{3\arrayrulewidth}
    Method & IJB-B & IJB-C\\
    \hline \hline
    ResNet50+SENet50  \cite{VGGFace2} & 80.0 & 84.1 \\
    Multicolumn  \cite{xie2018multicolumn} & 83.1 & 86.2\\
    P2SGrad  \cite{zhang2019p2sgrad} & - & 92.3\\
    Adacos  \cite{zhang2019adacos} & - & 92.4\\
    ArcFace-VGG2-R50  \cite{deng2019arcface} & 89.8 & 92.1\\
    ArcFace-MS1MV2-R100  \cite{deng2019arcface} & 94.2 & 95.6\\
   {CurricularFace-MS1MV2-R100}  \cite{huang2020curricularface}  & {94.8} & {96.1}\\
    % {AdaFace}  \cite{kim2022adaface} & {\underline{95.4}} & {96.}\\
    {MagFace-MS1MV2-R100}  \cite{meng2021magface}  & {94.5} & {96.0}\\
    \hline
    KappaFace-MS1MV2-R100 (\textbf{\texttt{Memory buffer}}) & \underline{95.1} & \underline{96.4} \\
        KappaFace-MS1MV2-R100 (\textbf{\texttt{Momentum encoder}}) & \textbf{95.3} & \textbf{96.6} \\
    \Xhline{3\arrayrulewidth}
    \end{tabular}%
}
\end{center}
\end{table*}



\begin{table*}[th!]
\begin{center}
\caption{{Verification performance, in terms of accuracy, compared with SOTA methods on MegaFace Challenge 1 using FaceScrub~\cite{ng2014data} as the probe set. The reported results are based on the refined data. Id corresponds to the rank 1 face identification accuracy with 1M distractors, whereas Ver refers to the face verification TAR (@FAR = $1e^{-6}$). The best performances are shown in bold, and the second best are underlined.}}
\label{tb:mf_exp}
\resizebox{.60\textwidth}{!}{%
    \begin{tabular}{ l|c|c} 
    \Xhline{3\arrayrulewidth}
    Method & Id & Ver\\
    \hline \hline
    AdaptiveFace \cite{liu2019adaptiveface} & 95.02 & 95.61\\
    P2SGrad  \cite{zhang2019p2sgrad} & 97.25 & -\\
    Adacos  \cite{zhang2019adacos} & 97.41 & -\\
    CosFace \cite{wang2018cosface} & 97.91 & 97.91\\
    MV-AM-Softmax-a \cite{wang2020mis} & 98.00 & 98.31\\
    ArcFace-MS1MV2-R100  \cite{deng2019arcface} & 98.35 & 98.48\\
    
    {CurricularFace-MS1MV2-R100}  \cite{huang2020curricularface}  & {98.71} &  {98.64}\\
    {MagFace-MS1MV2-R100}  \cite{meng2021magface}  & {97.78} & {98.10}\\
    \hline
    KappaFace-MS1MV2-R100 (\textbf{\texttt{Memory buffer}}) & \underline{98.77} & \textbf{98.91} \\
        KappaFace-MS1MV2-R100 (\textbf{\texttt{Momentum encoder}}) & \textbf{98.78} & \underline{98.83} \\
    \Xhline{3\arrayrulewidth}
    \end{tabular}%
}
\end{center}
\end{table*}


\begin{figure}[t!]
\centering
\includegraphics[width=8cm]{Figures/MS1MV2_MarginChanges.png}
\caption{Variation of margin values of~\SystemName~ + Momentum against training iterations. As stated, we fix the additive margin for the first couple of epochs. The blue line shows the average margin across identities.} 
\label{fig:margins}
\end{figure} 

\textbf{Results on MegaFace.} Next, we provide an evaluation result on the MegaFace Challenge 1. The gallery set of MegaFace consists of 1M images of 690K unique individuals, and the probe set has 100K photos of 530 subjects from FaceScrub. We report the results under a large training set protocol, where we train ResNet100 on MS1MV2. Note that the results reported are based on the refined MegaFace, where noisy labels are removed. Table \ref{tb:mf_exp} clearly shows that our method outperforms other state-of-the-art methods in both identification and verification tasks, where \SystemName{} trained with the memory buffer achieves 98.77 and 98.91, respectively.



\begin{comment}  %%%%%%%%%%%% COMMENT %%%%%%%%%%%%%%%%%%%

\subsection{Ablation Study}



\begin{figure*}[t!]
    \centering
    \subfloat[\centering \small{Histogram distribution of concentration ($\widehat{\kappa}_{c}$) values against number of classes.}]{{\includegraphics[width=11cm]{Figures/MS1MV2_ArcFacevsKappaFace_hist.png} }}%
    \qquad
    \subfloat[\centering \small{Normalized concentration values ($\widehat{\kappa}_{c}$) against number of samples ($n_c$).}]{{\includegraphics[width=6.0cm, height=4.0cm]{Figures/MS1MV2_ArcFacevsKappaFace_reorder_move.png} }}%
    \caption{Comparison of final concentration values of ArcFace and ~\SystemName. A, B, C, and D denote four examples of extreme classes shown in Fig. \ref{fig:illust_extreme}. Arrows indicate changes of relative concentrations from ArcFace to our KappaFace.}%
    \label{fig:arcfacevskappaface}%
\end{figure*} 

\begin{figure}[t!]
    \centering
    \subfloat[\centering \small{Class \textbf{A}: $\widehat{\kappa}_{c}=-2.30, n_{c}=432, \psi_c=0.69$} ]{{\includegraphics[width=7cm]{Figures/MS1MV2_Group A.png} }}%
    \qquad
    \subfloat[\centering \small{Class \textbf{B}: $\widehat{\kappa}_{c}=-2.30, n_{c}=9, \psi_c=0.74$}]{{\includegraphics[width=7cm]{Figures/MS1MV2_Group C.png} }}%
    \qquad
    \subfloat[\centering \small{Class \textbf{C}: $\widehat{\kappa}_{c}=5.21, n_{c}=4, \psi_c=0.76$}]{{\includegraphics[width=7cm]{Figures/MS1MV2_Group D.png} }}%
    \qquad
    \subfloat[\centering \small{Class \textbf{D}: $\widehat{\kappa}_{c}=-0.10, n_{c}=128, \psi_c=0.74$} ]{{\includegraphics[width=7cm]{Figures/MS1MV2_Group B.png} }}%
    \caption{Examples from four extreme classes varying from small to high concentration ($\widehat{\kappa}_{c}$), and from underrepresented to over represented ($n_c$) ones.}%
    \label{fig:illust_extreme}%
\end{figure}

\end{comment} %%%%%%%%%%%% COMMENT %%%%%%%%%%%%%%%%%%%


\textbf{Probabilistic models with smaller backbone. } In this study, we compare our approach with SOTA probabilistic deep face models, namely ArcFace-PFE-G \cite{shi2019probabilistic}, ArcFace-SCF \cite{li2021spherical}, and {LDAM-DRW}~\cite{cao2019learning},  {with a smaller backbone (ResNet34). We note that LDAM-DRW is proposed to address imbalanced datasets in classification problems; however, as it is closely related to our work, we fine tuned it for the deep face embedding model.} As shown in Table \ref{tb:small_bb_exp}, all three probabilistic models present a considerable improvement upon the ArcFace baseline across all the experimental datasets. Our \SystemName, on the other hand, consistently outperforms the counterparts by a decent margin. Notably, it achieves a staggering $99.82 \%$ accuracy on LFW dataset, which is comparable to the results obtained from ResNet100.

\textbf{Hyper-parameter fine-tuning. }In this study, we use ResNet100 with the momentum encoder to analyze how various settings of $T$ and $m_0$ affect ~\SystemName~ on the MS1MV2. We select LFW, CFP-FP, AgeDB, IJB-B and IJB-C datasets for our experiments. 
As we can examine from  Table \ref{tb:ablation}, the optimal setting observed in our series of experiments was $m_{0} = 0.8$, and $T = 0.4$. However, we would also like to emphasize that some other settings work better on individual datasets. For example, ~\SystemName~ with  $m_{0} = 0.7$ and $T = 0.4$ works better on CFP-FP and AgeDB yet we observe the performance drop on IJB-B and IJB-C datasets. 
Our proposed ~\SystemName~ shows the robustness and improvements over the fixed margin used by the ArcFace loss.  Table ~\ref{tb:ablation} demonstrates that our proposed method outperforms ArcFace in all the selected evaluation datasets. In addition, Figure \ref{fig:margins} demonstrates how margin values change throughout the training process, whereas ArcFace utilizes a fixed margin value of $0.5$, which is an optimal value reported by the authors \cite{deng2019arcface}. Although the values fluctuate, especially the maximum value, we observe that the mean value tends to stay around $0.55$. 

{\textbf{Contribution of class concentration and population weights}. We ablate along the hyper-parameter $\gamma$ with MS1MV2 dataset and ResNet34 backbone. From the results in Table} \ref{tb:ablate_gamma}, {we note that at any values of $\gamma$ our model can substantially outperform the baseline ArcFace} \cite{deng2019arcface}{. Moreover, with $\gamma=0.7$, as we suggested, }\SystemName{}{ obtains the optimal performance.} {The table also shows that both terms $w_{c}^{k}$ and $w_{c}^{s}$ contribute to our final results. Note that only $w_{c}^{k}$ changes throughout the training, hence one may replace or drop $w_{c}^{s}$. However, we believe it encourages to learn under-represented categories in case concentration values for well-represented and poorly-represented identities are equal.}



\begin{table*}[th!]
\begin{center}
\caption{Ablation study on verification performance with ResNet34 + Momentum Encoder on LFW, CFP-FP, AgeDB, CALFW and CPLFW.}
\label{tb:small_bb_exp}
\resizebox{.80\textwidth}{!}{%
    \begin{tabular}{ l|c|c|c|c|c} 
    \Xhline{3\arrayrulewidth}
    Method & LFW & CFP-FP & CPLFW & AgeDB & CALFW \\
    \hline \hline
    ArcFace  \cite{deng2019arcface} & 99.68 & 94.04 & 89.30 &  96.60 & 95.00\\
    ArcFace-PFE-G   \cite{shi2019probabilistic} & 99.71 & 94.19 & 89.90 & 96.70 & 95.49 \\
    ArcFace-SCF   \cite{li2021spherical} & 99.73 & 94.87 & 90.62 & 97.16 & 95.79 \\
    {LDAM-DRW} \cite{cao2019learning} & {99.80} & {97.41} &{91.73} & {97.72} & {95.95}\\
    \hline
        KappaFace  & \textbf{99.82} & \textbf{97.57} & \textbf{92.00} & \textbf{98.02} & \textbf{96.13}\\
    \Xhline{3\arrayrulewidth}
    \end{tabular}
    }
\end{center}
\end{table*}

\begin{table*}[t!]
\begin{center}
\caption{{Ablation studies on our hyperparameters with ResNet100 + Momentum Encoder, where the performance gains are shown in green, and drops in red compared to the optimal setting (shown in bold).}}
\label{tb:ablation}
\resizebox{.76\textwidth}{!}{%
    \begin{tabular}{ c|c|c|c|c|c|c } 
    \Xhline{3\arrayrulewidth}
    \multicolumn{2}{c|}{Hyper-parameters}  & \multicolumn{5}{c}{Datasets} \Bstrut\\ 
    \hline
    $m_0$ & $T$ & LFW & CFP-FP & AgeDB & IJB-B & IJB-C \Tstrut\\
    \hline \hline
    0.8 & 0.4 & \textbf{99.83} & \textbf{98.60} & \textbf{98.35} & \textbf{95.3} & \textbf{96.6}\Tstrut\\
    \hline
    0.8 & \textit{0.3} & 99.83 & 98.63 \textcolor{green}{(+0.03)} &  98.32 \textcolor{red}{(-0.03)} & 95.17 \textcolor{red}{(-0.13)} & 96.44 \textcolor{red}{(-0.16)}\Tstrut\\
    0.8 & \textit{0.5} & 99.83 & 98.63 \textcolor{green}{(+0.03)} & 98.35 &  95.29  \textcolor{red}{(-0.01)} & 96.53 \textcolor{red}{(-0.07)}\\
    \hline
    \textit{0.7} & 0.4  & 99.83 & 98.71 \textcolor{green}{(+0.11)} & 98.40 \textcolor{green}{(+0.05)} &  95.10 \textcolor{red}{(-0.20)} & 96.53  \textcolor{red}{(-0.07)}\Tstrut\\
    \textit{0.9} & 0.4 & 99.83 & 98.51 \textcolor{red}{(-0.09)} & 98.35 & 95.24 \textcolor{red}{(-0.06)} & 96.50 \textcolor{red}{(-0.10)}\Bstrut\\
    \Xhline{3\arrayrulewidth}
    \end{tabular}%
}
\end{center}
\end{table*}

\begin{table*}[th!]
\begin{center}
\caption{{Ablation study on $\gamma$ with ResNet34 + Momentum Encoder on LFW, CFP-FP, AgeDB, CALFW and CPLFW.}}
\label{tb:ablate_gamma}
\resizebox{.62\textwidth}{!}{%
    \begin{tabular}{ l|c|c|c|c|c } 
    \Xhline{3\arrayrulewidth}
    $\gamma$ & LFW & CFP-FP & CPLFW & AgeDB & CALFW  \\
    \hline \hline
    ArcFace  \cite{deng2019arcface} & 99.68 & 94.04 & 89.30 &  96.60 & 95.00 \\
    \hline
    0.0   & {99.82} & {96.29} & {91.13} & \textbf{98.03} &{96.07}\\
    0.3    & {99.82} & {96.72} & {91.71} & {97.95} & {96.07}\\
    0.5    & {99.82} & {97.04} & {91.53} & {97.85} & {96.05}\\
    \rowcolor{Gray}0.7  & \textbf{99.82} & \textbf{97.57} & {92.00} & {98.02} & \textbf{96.13} \\
    1.0  & {99.80} & {97.57} & \textbf{92.10} & {97.97} & {96.12} \\
    \Xhline{3\arrayrulewidth}
    \end{tabular}
    }
\end{center}
\end{table*}


\begin{figure*}[t!]
\centering
\includegraphics[width=6.0in]{Figures/kappa_illus.png}
\caption{\textbf{Identity vs. concentration value.} Each column corresponds to an identity, with 4 random samples provided, and their $\kappa$s are sorted in ascending order from left to right. {We demonstrate that $\kappa$ can be affected by how noisy, diverse or available samples are.}} 
\label{fig:kappa_illustration}
\end{figure*} 
\textbf{Qualitative analysis}. We provide Figure \ref{fig:kappa_illustration} to demonstrate that the $\kappa$ value can represent a class learning difficulty in the training dataset, MS1MV2. The class samples in the left-most column are noisy and have different qualities; hence its $\kappa$ is the smallest. Moving from the left to right-hand side column, identities vary less in terms of age and the sample quality gradually improves, indicated by the increasing $\kappa$. Finally, we also perform an ablation study on the IJB-C dataset to show the advantages of our proposed \SystemName{} over the baseline ArcFace model in the verification task. As shown in Figure \ref{fig:pos_pairs} and Figure \ref{fig:neg_pairs}, our method, \SystemName, efficiently represents the positive images with higher cosine similarity values compared to {the} ArcFace. Meanwhile, for the negative pairs, the \SystemName{} can push their representations away farther apart, showing through the smaller similarity values. 

\begin{figure*}[t!]
\centering
\includegraphics[width=6.8in]{Figures/postive_pairs.pdf}
\caption{\textbf{Positive pairs from IJB-C dataset.} $\cos \theta$ is the cosine distance of a verification pair $x_1$ and $x_2$. The lower the $\cos \theta$, the more likely that the model has larger false positive rate. Thus, the green values indicate the improvements over ArcFace. } 
\label{fig:pos_pairs}
\end{figure*}
\begin{figure*}[t!]
\centering
\includegraphics[width=6.8in]{Figures/negative_pairs.pdf}
\caption{\textbf{Negative pairs from IJB-C dataset.} $\cos \theta$ is the cosine distance of a verification pair $x_1$ and $x_2$. The greater the $\cos \theta$, the more likely that the model has larger false negative rate. Thus, the green values indicate the improvements over ArcFace.} 
\label{fig:neg_pairs}
\end{figure*}

% Next, we provide Fig. \ref{fig:arcfacevskappaface} that presents the distribution of the final concentration values for both ArcFace and ~\SystemName. As it can be observed from the sub-figure \emph{(a)}, ~\SystemName achieves staggeringly greater concentration values comparing to ArcFace. Moreover, the  sub-figure \emph{(b)} also shows that the normalized concentration values of ArcFace can greatly deviate from the mean value. Therefore, this clearly demonstrates that applying the same margin to all classes leads to biased decision boundaries.
% Under our training scheme of ~\SystemName, margins of easy classes in ArcFace are relaxed by increasing normalized concentrations (\textit{rightwards  arrows}), and margins of hard classes are intensified (\textit{leftwards arrows}).
%low concentration - large population (\textbf{A}),  high concentration - large population (\textbf{B}),  low concentration - small population (\textbf{C}),  and low concentration - small population (\textbf{D}),

%  From Fig. \ref{fig:arcfacevskappaface}, we select four extreme classes and show their samples in Fig. \ref{fig:illust_extreme} to explain the fundamental causes of the differences. As one may observe samples of the class \textbf{A}, which were collected with a wide range of angles, ages and resolutions, produce a concentration of 2.30 standard deviations smaller than the mean yet there are 432 samples available.  Class \textbf{B} contains only 9 samples, containing somewhat noisy images, hence the concentration value turned out to be low. On the other hand, Class \textbf{C} includes only four high-quality photos having a small variance in terms of facial angles and ages. Therefore, the resulting concentration value is very high. However, from our observation, class \textbf{D} obtains only augmentation version of one single photo. Acting differently with ArcFace, out KappaFace relaxes the constraint on class \textbf{D}'s concentration since it contains sufficient number of augmented photos. Although there is only one actual sample of a person's face, its concentration value does not deviate from the mean much, whereas another easy class \textbf{C} achieves considerably greater concentration value due to its low population. From this observation, one may explore further steps on pre-processing the training data to achieve better feature representations; however, it is out of scope of our paper and we leave it for future works.


